Cloudprofiler: TSC-based inter-node profiling and high-throughput data ingestion for cloud streaming workloads

To conduct real-time analytics computations, big data stream processing engines are required to process unbounded data streams at millions of events per second. However, current streaming engines exhibit low throughput and high tuple processing latency. Performance engineering is complicated by the fact that streaming engines constitute complex distributed systems consisting of multiple nodes in the cloud. A profiling technique is required that is capable of measuring time durations at high accuracy across nodes. Standard clock synchronization techniques such as the network time protocol (NTP) are limited to millisecond accuracy, and hence cannot be used. We propose a profiling technique that relates the time-stamp counters (TSCs) of nodes to measure the duration of events in a streaming framework. The precision of the TSC relation determines the accuracy of the measured duration. The TSC relation is conducted in quiescent periods of the network to achieve accuracy in the tens of microseconds. We propose a throughput-controlled data generator to reliably determine the sustainable throughput of a streaming engine. To facilitate high-throughput data ingestion, we propose a concurrent object factory that moves the deserialization overhead of incoming data tuples off the critical path of the streaming framework. The evaluation of the proposed techniques within the Apache Storm streaming framework on the Google Compute Engine public cloud shows that data ingestion increases from $700$ $\text{k}$ to $4.68$ $\text{M}$ tuples per second, and that time durations can be profiled at a measurement accuracy of $92$ $\mu\text{s}$, which is three orders of magnitude higher than the accuracy of NTP, and one order of magnitude higher than prior work.

==> figures/CP_method_ratio.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Commands gobble following space
% https://texfaq.org/FAQ-xspace
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\usetikzlibrary{math}
\def\RectW{252.94499}%
\def\Offset{16}%
\def\RectH{143+\Offset}%
\def\TickH{6}%
\def\SmallTickH{2}%
\def\LongTickH{5}%
\def\YofNodeA{44+\Offset}%
\def\YofNodeB{124+\Offset}%
\def\PeriodA{2.930}%
\def\PeriodB{5.125}% 0,1,...,48
\newcommand{\TSCv}[2]{T-c#1#2}%
\newcommand{\STRv}[2]{S-c#1#2}%
%
\newcommand{\DrawTick}[3]% name, position,yshift
{
  \coordinate (#1) at (#2);
  \coordinate[yshift=#3] (#1-top) at (#1);
  \path [tick3] (#1.north) -- (#1-top);
}%
%
\begin{tikzpicture}[
  %fill=blue!5
  rect0/.style={solid,thick,inner sep=3pt,minimum width=40pt},
  dot0/.style={draw=black!0,solid,thick},
  guide/.style={draw=black,dashed,line join=round,line width=0.1pt},
  line0/.style={draw=black,solid,line join=round,line width=1pt},
  tick0A/.style={draw,minimum height=\TickH,minimum width=0pt,inner sep=0pt,line
  width=\pgflinewidth,yshift=3pt,xshift=-10pt},
  % tick1A: distanced at a period of C^A
  tick1A/.style={draw,minimum height=\TickH,minimum width=0pt,inner sep=0pt,line
  width=\pgflinewidth,xshift=-18pt},
  tick0B/.style={draw,minimum height=\TickH,minimum width=0pt,inner sep=0pt,line
   width=\pgflinewidth,yshift=3pt,xshift=-6pt},
  tick1B/.style={draw,minimum height=\TickH,minimum width=0pt,inner sep=0pt,line
  width=\pgflinewidth,xshift=-10pt},
  tickP/.style={draw,minimum height=\TickH,minimum width=0pt,inner sep=0pt,line
  width=\pgflinewidth,yshift=-16pt},
  tick/.style={draw,minimum height=\TickH,minimum width=0pt,inner sep=0pt,line
  width=\pgflinewidth,cap=rect},
  tick2/.style={draw=red,line width=\pgflinewidth,cap=rect},
  tick3/.style={draw,line width=\pgflinewidth,cap=rect},
  textA/.style={align=center,yshift=16pt},
  textB/.style={align=center,yshift=-16pt},
  mynode/.style 2 args={inner sep=0pt,outer sep=0pt,fit=(#1) (#2),
  postaction={on layer=back,fill,yellow},
  postaction={on layer=back,draw,yellow}},
  myarrow/.style={double arrow, fill=red!100, anchor=base, align=center,text
  width=27pt},
  y=1pt, x=1pt, inner sep=0pt, outer sep=0pt,align=center]
  %\tikzstyle{guide0}=[draw=black,dashed,line join=round,line width=0.1pt]
  %\tikzstyle{tick0}=[draw,minimum height = 1pt,minimum width=10pt,inner sep=0pt]
  %\tikzstyle{node0}=[draw=black,line join=round,line width=0.1pt]
  \tikzstyle{transition}=[rectangle,draw=black!50,fill=black!20,thick]
\begin{scope}
\path[clip] (0.00, 0.00) rectangle(\RectW, \RectH);


  %\path[guide] (0.00, 0.00) rectangle(\RectW, \RectH);
  %\path[node0] (0, 50) rectangle(50, 30);


  %\path[rect0] (0, 50) rectangle(35, 25);
  %\path[guide] (0,\RectH) -- (\RectW,\RectH);
  %\path[guide] (0,0) -- (\RectW,0);



  %\path[textA] (0,0) node[above right] (text6971) {Hello};
  \coordinate (AStarts) at (0, \YofNodeA);
  \coordinate (BStarts) at (0, \YofNodeB);
  \coordinate (AEnds) at (\RectW,\YofNodeA);
  \coordinate (BEnds) at (\RectW,\YofNodeB);
  \node[rect0,yshift=-15pt,xshift=4pt] (NodeA) [above of=AEnds,left] {TSC~\TSC{A}};
  \node[rect0,yshift=15pt,xshift=4pt] (NodeB) [below of=BEnds,left] {TSC~\TSC{B}};
  \path [>=Latex,->,draw,line width=\pgflinewidth,name path=TimelineA] (AStarts) -- (AEnds.west);
  \path [>=Latex,->,draw,line width=\pgflinewidth,name path=TimelineB] (BStarts) -- (BEnds.west);

  %Newtonian Time
  \coordinate[yshift=-48pt] (C-NewtonTime-west) at (AStarts);
  \coordinate[yshift=-48pt] (C-NewtonTime-east) at (AEnds);
  \path [>=Latex,->,draw=yellow!75!magenta,line width=2.0\pgflinewidth,name path=NewtonTime]
  (C-NewtonTime-west) -- (C-NewtonTime-east) coordinate[pos=0.808,yshift=-8pt] (C-NewtonTime);
  \node (S-NewtonTime) at (C-NewtonTime) {Newtonian Time};

  % All ticks of TSC~C^A
  \edef\X{0}
  \edef\name{}
  \foreach \x in {0,1,...,83}
  {
    \xdef\name{\TSCv{\x}{A}}
    \pgfmathparse{\X+\PeriodA}
    \xdef\X{\pgfmathresult}
    \coordinate (\name) at (\X, \YofNodeA);
    \coordinate[yshift=\SmallTickH] (\name-top) at (\name);
    \path [tick3] (\name.north) -- (\name-top);
  }

  % All ticks of TSC~C^B
  \edef\X{0}
  \edef\name{}
  \foreach \x in {0,1,...,47}
  {
    \xdef\name{\TSCv{\x}{B}}
    \pgfmathparse{\X+\PeriodB}
    \xdef\X{\pgfmathresult}
    \coordinate (\name) at (\X, \YofNodeB);
    \coordinate[yshift=\SmallTickH] (\name-top) at (\name);
    \path [tick3] (\name.north) -- (\name-top);
  }

  % MRTT#1 on Node A
  \DrawTick{\TSCv{i}{A}}{\TSCv{1}{A}}{\LongTickH}
  \node[textA] (\STRv{i}{A}) [below of=\TSCv{i}{A}] {\Tick{c}{i}{A}};
  \DrawTick{\TSCv{k}{A}}{\TSCv{27}{A}}{\LongTickH}
  \node[textA] (\STRv{k}{A}) [below of=\TSCv{k}{A}] {\Tick{c}{k}{A}};
  % Uncertainty due to MRTT#1
  \coordinate[xshift=4pt,yshift=-6pt] (middle0) at ($(\STRv{i}{A}.south)!0.5!(\STRv{k}{A}.south)$) {};
  \draw [decorate,decoration={brace,amplitude=6pt,mirror,raise=1ex},line
  width=1.5\pgflinewidth] (\STRv{i}{A}.south) -- (\STRv{k}{A}.south);
  \node[textA] (\STRv{i}{A}-ckA) [below of=middle0]
  {$\tk[g]{j}{A}=\best{j}{A}\pm\error{c}{j}{A}$};

  % MRTT#1 on Node B
  \DrawTick{\TSCv{j}{B}}{\TSCv{3}{B}}{\LongTickH}
  \node[textB] (\STRv{j}{B}) [above of=\TSCv{j}{B}] {\Tick{c}{j}{B}};
  % A light gray box for MRTT#1
  \path[name path=MRTT1-lower-bound]
  (\TSCv{i}{A}.south) -- ($(\TSCv{0}{B}.south)!(\TSCv{i}{A})!(\TSCv{1}{B}.south)$) coordinate[pos=0.00]
  (C-MRTT1-bottom-left);
  \path[name path=MRTT1-upper-bound]
  (\TSCv{k}{A}.south) -- ($(\TSCv{0}{B}.south)!(\TSCv{k}{A})!(\TSCv{1}{B}.south)$) coordinate[pos=1.00]
  (C-MRTT1-top-right);
  \node[fit=(C-MRTT1-bottom-left) (C-MRTT1-top-right),postaction={on
  layer=back,fill,lightgray!30!white},
  postaction={on layer=back,draw,lightgray!30!white}] (MRTT1-box) {};
  % MRTT#1 Label
  \node[above left,rotate=90] (S-MRTT1) at (C-MRTT1-top-right) {\MinRTT{1}};

  % Write a label ``error'', its left and right boundings, and the red arrow
  % Lower-bound between cjA and cjA-best
  \path[draw,dotted,cap=rect,line width=1.25\pgflinewidth,name path=true-bound]
  (\TSCv{j}{B}) -- ($(\TSCv{0}{A})!(\TSCv{j}{B})!(\TSCv{1}{A})$)
  coordinate[pos=0.85] (C-true-bound-midway);
  \coordinate (\TSCv{j}{A}) at ($(\TSCv{0}{A}.south)!(\TSCv{j}{B})!(\TSCv{1}{A}.south)$);
  \node[textA] (\STRv{j}{A}) [below of=\TSCv{j}{A}] {\Tick{c}{j}{A}};
  % Upper-bound between cjA and cjA-best
  \coordinate (\TSCv{j}{A}-best) at ($(\TSCv{i}{A}.south)!0.5!(\TSCv{k}{A}.south)$);
  \node[textA] (\STRv{j}{A}-best) [below of=\TSCv{j}{A}-best] {$\hat{c}_{j}^{A}$};
  \coordinate (\TSCv{j}{B}-best) at ($(\TSCv{0}{B}.south)!(\TSCv{j}{A}-best)!(\TSCv{1}{B}.south)$);
  \node[textB,text=cyan!64!magenta!95!black] (\STRv{j}{B}-best) [above of=\TSCv{j}{B}-best] {$\hat{c}_{j}^{B}$};
  \path[draw,dotted,cap=rect,line width=1.25\pgflinewidth,name path=best-bound]
  (\TSCv{j}{B}-best) -- (\TSCv{j}{A}-best)
  coordinate[pos=0.85] (C-best-bound-midway);
  \path[>=Latex,<->,draw=red,line width=\pgflinewidth]
  (C-true-bound-midway) -- (C-best-bound-midway) coordinate[pos=0.5]
  (C-error-arrow-midway);
  \node[yshift=-20pt] (S-error) [above of=C-error-arrow-midway]
  {$\mathit{error}$};

  % Ideal round-trip of MRTT#1
  \path[draw=cyan!64!magenta!95!black,dashed,cap=rect,>=Latex,->,line width=\pgflinewidth] (\TSCv{i}{A}.south) -- (\TSCv{j}{B}-best.south);
  \path[draw=cyan!64!magenta!95!black,dashed,cap=rect,>=Latex,->,line width=\pgflinewidth] (\TSCv{j}{B}-best.south) -- (\TSCv{k}{A}.south);
  % Round-trip of MRTT#1
  \path[draw,>=Latex,->,solid,line width=1.25\pgflinewidth] (\TSCv{i}{A}.south) -- (\TSCv{j}{B}.south);
  \path[draw,>=Latex,->,solid,line width=1.25\pgflinewidth] (\TSCv{j}{B}.south) -- (\TSCv{k}{A}.south);

  % An inter-node event on Node A
  \DrawTick{\TSCv{x}{A}}{\TSCv{36}{A}}{\LongTickH}
  \node[textA,text=blue] (\STRv{x}{A}) [below of=\TSCv{x}{A}] {\Tick{c}{x}{A}};
  \node[text=blue,xshift=-10pt] (S-e1) [right of=\STRv{x}{A}] {$=e_{1}$};

  % An inter-node event on Node B
  \DrawTick{\TSCv{y}{B}}{\TSCv{28}{B}}{\LongTickH}
  \node[textB,text=red] (\STRv{y}{B}) [above of=\TSCv{y}{B}] {\Tick{c}{y}{B}};
  \node[text=red,xshift=-10pt] (S-e2) [right of=\STRv{y}{B}] {$=e_{2}$};

  % Approximation of C_y^B to C_y^A
  \coordinate (\TSCv{y}{A}) at ($(\TSCv{0}{A}.south)!(\TSCv{y}{B})!(\TSCv{1}{A}.south)$);
  \node[textA,text=red] (\STRv{y}{A}) [below of=\TSCv{y}{A}] {\Tick{c}{y}{A}};

  % MRTT#2 on Node A
  \DrawTick{\TSCv{l}{A}}{\TSCv{57}{A}}{\LongTickH}
  \node[textA] (\STRv{l}{A}) [below of=\TSCv{l}{A}] {\Tick{c}{l}{A}};
  \DrawTick{\TSCv{n}{A}}{\TSCv{72}{A}}{\LongTickH}
  \node[textA] (\STRv{n}{A}) [below of=\TSCv{n}{A}] {\Tick{c}{n}{A}};
  % Uncertainty due to MRTT#2
  \coordinate[yshift=-6pt] (middle0) at ($(\STRv{l}{A}.south)!0.5!(\STRv{n}{A}.south)$) {};
  \draw [decorate,decoration={brace,amplitude=6pt,mirror,raise=1ex},line
  width=1.5\pgflinewidth] (\STRv{l}{A}.south) -- (\STRv{n}{A}.south);
  \node[textA] (\STRv{l}{A}-cnA) [below of=middle0] {\Tick{c}{m}{A}};

  % MRTT#2 on Node B
  \DrawTick{\TSCv{m}{B}}{\TSCv{40}{B}}{\LongTickH}
  \node[textB] (\STRv{m}{B}) [above of=\TSCv{m}{B}] {\Tick{c}{m}{B}};
  % A light gray box for MRTT#2
  \path[name path=MRTT2-lower-bound]
  (\TSCv{l}{A}.south) -- ($(\TSCv{0}{B}.south)!(\TSCv{l}{A})!(\TSCv{1}{B}.south)$) coordinate[pos=0.00]
  (C-MRTT2-bottom-left);
  \path[name path=MRTT2-upper-bound]
  (\TSCv{n}{A}.south) -- ($(\TSCv{0}{B}.south)!(\TSCv{n}{A})!(\TSCv{1}{B}.south)$) coordinate[pos=1.00]
  (C-MRTT2-top-right);
  \node[fit=(C-MRTT2-bottom-left) (C-MRTT2-top-right),postaction={on
  layer=back,fill,lightgray!30!white},
  postaction={on layer=back,draw,lightgray!30!white}] (MRTT2-box) {};
  \coordinate (C-MRTT2-top-left) at ($(\TSCv{0}{B}.south)!(\TSCv{l}{A})!(\TSCv{1}{B}.south)$);
  % MRTT#2 Label
  \node[below left,rotate=90] (S-MRTT2) at (C-MRTT2-top-left) {\MinRTT{2}};

  % Draw duration (a yellow box)
  \path[name path=duration-lower-bound]
  (\TSCv{x}{A}.south) -- ($(\TSCv{0}{B}.south)!(\TSCv{x}{A})!(\TSCv{1}{B}.south)$) coordinate[pos=0.15]
  (C-duration-lower-midway);
  \path[name path=duration-upper-bound]
  ($(\TSCv{0}{A}.south)!(\TSCv{y}{B})!(\TSCv{1}{A}.south)$) -- (\TSCv{y}{B}.south) coordinate[pos=0.15]
  (C-duration-upper-midway);
  \node[fit=(\TSCv{x}{A}.south) (\TSCv{y}{B}.north),postaction={on
  layer=back,fill,yellow},
  postaction={on layer=back,draw,yellow}] (duration-box) {};

  %>=triangle 45
  %>=Latex
  \path[>=Latex,<->,draw=red,line width=\pgflinewidth]
  (C-duration-lower-midway) -- (C-duration-upper-midway) coordinate[pos=0.5]
  (C-duration-arrow-midway);
  \node[yshift=-20pt] (S-duration-01) [above of=C-duration-arrow-midway]
  %{$d_{\left(c_{x}^{A},c_{y}^{B}\right)}$};
  {\DurSym{x}{y}{A}};
  %{\NewDuration{event}};
  \node[yshift=-16pt] (S-duration-02) [above of=S-duration-01] {duration};

  % Round-trip of MRTT#2
  %\path[draw,>=Latex,->,solid,line width=1.25\pgflinewidth] (\TSCv{i}{A}.south) -- (\TSCv{j}{B}.south);
  \path[draw,>=Latex,->,solid,line width=1.25\pgflinewidth] (\TSCv{l}{A}.south) -- (\TSCv{m}{B}.south);
  \path[draw,>=Latex,->,solid,line width=1.25\pgflinewidth] (\TSCv{m}{B}.south) -- (\TSCv{n}{A}.south);

  % yellow box
\end{scope}

\end{tikzpicture}


==> figures/CP_method_ratio_2.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Commands gobble following space
% https://texfaq.org/FAQ-xspace
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\usetikzlibrary{math}
\def\RectW{252.94499}%
\def\OffsetX{10}%
\def\OffsetY{16}%
\def\RectH{143+\OffsetY}%
\def\TickH{6}%
\def\SmallTickH{2}%
\def\LongTickH{2}%
\def\GlobalX{\OffsetX}%
% Case A
\def\YofNodeBCaseA{127+\OffsetY}%
\def\YofNodeACaseA{107+\OffsetY}%
% Case B
\def\YofNodeCCaseB{73+\OffsetY}%
\def\YofNodeBCaseB{53+\OffsetY}%
% Case C
\def\YofNodeCCaseC{20+\OffsetY}%
\def\YofNodeACaseC{0+\OffsetY}%
%
\def\PeriodA{2.930}%
\def\PeriodB{5.125}%
\def\PeriodC{2.255}%
\def\MaxTksA{79}%
\def\MaxTksB{45}%
\def\MaxTksC{103}%
%
\newcommand{\TSCv}[2]{T-c#1#2}%
\newcommand{\STRv}[2]{S-c#1#2}%
%
\newcommand{\DrawTick}[3]% name, position,yshift
{
  \coordinate (#1) at (#2);
  \coordinate[yshift=#3] (#1-top) at (#1);
  \path [tick3,draw] (#1.north) -- (#1-top);
}%
%
\begin{tikzpicture}[
  %fill=blue!5
  rect0/.style={solid,thick,inner sep=3pt,minimum width=40pt},
  dot0/.style={draw=black!0,solid,thick},
  guide/.style={draw=black,dashed,line join=round,line width=0.1pt},
  line0/.style={draw=black,solid,line join=round,line width=1pt},
  tick0A/.style={draw,minimum height=\TickH,minimum width=0pt,inner sep=0pt,
    line width=\pgflinewidth,yshift=3pt,xshift=-10pt},
  % tick1A: distanced at a period of C^A
  tick1A/.style={draw,minimum height=\TickH,minimum width=0pt,inner sep=0pt,
    line width=\pgflinewidth,xshift=-18pt},
  tick0B/.style={draw,minimum height=\TickH,minimum width=0pt,inner sep=0pt,
    line width=\pgflinewidth,yshift=3pt,xshift=-6pt},
  tick1B/.style={draw,minimum height=\TickH,minimum width=0pt,inner sep=0pt,
    line width=\pgflinewidth,xshift=-10pt},
  tickP/.style={draw,minimum height=\TickH,minimum width=0pt,inner sep=0pt,
    line width=\pgflinewidth,yshift=-16pt},
  tick/.style={draw,minimum height=\TickH,minimum width=0pt,inner sep=0pt,
    line width=\pgflinewidth,cap=rect},
  tick2/.style={draw=red,line width=\pgflinewidth,cap=rect},
  tick3/.style={line width=\pgflinewidth,cap=rect},
  textA/.style={align=center,yshift=19pt},
  textB/.style={align=center,yshift=-19pt},
  mynode/.style 2 args={inner sep=0pt,outer sep=0pt,fit=(#1) (#2),
  postaction={on layer=back,fill,yellow},
  postaction={on layer=back,draw,yellow}},
  myarrow/.style={double arrow, fill=red!100, anchor=base, align=center,text
  width=27pt},
  mrttarrow/.style={draw,>=Latex,->,solid,line width=1.25\pgflinewidth},
  mrttarrow2/.style={draw=cyan!64!magenta!95!black,dashed,cap=rect,>=Latex,->,
    line width=\pgflinewidth},
  timeline/.style={>=Latex,->,draw,line width=\pgflinewidth},
  y=1pt, x=1pt, inner sep=0pt, outer sep=0pt,align=center]
  %\tikzstyle{guide0}=[draw=black,dashed,line join=round,line width=0.1pt]
  %\tikzstyle{tick0}=[draw,minimum height = 1pt,minimum width=10pt,inner sep=0pt]
  %\tikzstyle{node0}=[draw=black,line join=round,line width=0.1pt]
  \tikzstyle{transition}=[rectangle,draw=black!50,fill=black!20,thick]
\begin{scope}
\path[clip] (0.00, 0.00) rectangle(\RectW, \RectH);

  %% GUIDE BOX %%
  %\path[guide] (0.00, 0.00) rectangle(\RectW, \RectH);

  \coordinate (AStarts) at (\GlobalX, \YofNodeACaseA);
  \coordinate (BStarts) at (\GlobalX, \YofNodeBCaseA);
  \coordinate (AEnds) at (\RectW,\YofNodeACaseA);
  \coordinate (BEnds) at (\RectW,\YofNodeBCaseA);
  \node[rect0,xshift=-5pt] (NodeA) at (AStarts.north) {A};
  \node[rect0,xshift=-5pt] (NodeB) at (BStarts.north) {B};
  \path [timeline,name path=TimelineA] (AStarts) -- (AEnds.west);
  \path [timeline,name path=TimelineB] (BStarts) -- (BEnds.west);

  % All ticks of TSC~C^A
  \edef\X{\GlobalX}
  \edef\name{}
  \foreach \x in {0,1,...,\MaxTksA}
  {
    \xdef\name{\TSCv{\x}{A}}
    \pgfmathparse{\X+\PeriodA}
    \xdef\X{\pgfmathresult}
    \coordinate (\name) at (\X, \YofNodeACaseA);
    \coordinate[yshift=\SmallTickH] (\name-top) at (\name);
    \path [tick3] (\name.north) -- (\name-top);
  }

  % All ticks of TSC~C^B
  \edef\X{\GlobalX}
  \edef\name{}
  \foreach \x in {0,1,...,\MaxTksB}
  {
    \xdef\name{\TSCv{\x}{B}}
    \pgfmathparse{\X+\PeriodB}
    \xdef\X{\pgfmathresult}
    \coordinate (\name) at (\X, \YofNodeBCaseA);
    \coordinate[yshift=\SmallTickH] (\name-top) at (\name);
    \path [tick3] (\name.north) -- (\name-top);
  }

  % draw MinRTT
  {
    \xdef\nA{A}
    \xdef\nB{B}
    \xdef\tA{i}
    \xdef\tB{j}
    \xdef\tC{k}
    \xdef\cA{1}
    \xdef\cB{3}
    \xdef\cC{15}

    \DrawTick{\TSCv{\tA}{\nA}}{\TSCv{\cA}{\nA}}{\LongTickH}
    \node[textA] (\STRv{\tA}{\nA}) [below of=\TSCv{\tA}{\nA}]
    {\Tick{c}{\tA}{\nA}};
    \DrawTick{\TSCv{\tC}{\nA}}{\TSCv{\cC}{\nA}}{\LongTickH}
    \node[textA] (\STRv{\tC}{\nA}) [below of=\TSCv{\tC}{\nA}] {\Tick{c}{\tC}{\nA}};
    \DrawTick{\TSCv{\tB}{\nB}}{\TSCv{\cB}{\nB}}{\LongTickH}
    \node[textB] (\STRv{\tB}{\nB}) [above of=\TSCv{\tB}{\nB}] {\Tick{c}{\tB}{\nB}};
    %
    \path (\TSCv{\tA}{\nA}.south) --
    ($(\TSCv{0}{\nB}.south)!(\TSCv{\tA}{\nA})!(\TSCv{1}{\nB}.south)$) coordinate[pos=0]
    (C-MRTT1-bottom-left);
    \path (\TSCv{\tC}{\nA}.south) --
    ($(\TSCv{0}{\nB}.south)!(\TSCv{\tC}{\nA})!(\TSCv{1}{\nB}.south)$) coordinate[pos=1]
    (C-MRTT1-top-right);
    \node[fit=(C-MRTT1-bottom-left) (C-MRTT1-top-right),
    postaction={on layer=back,fill,lightgray!30!white},
    postaction={on layer=back,draw,lightgray!30!white}] (MRTT1-box) {};
    % Round-trip of MRTT#1
    \path[mrttarrow] (\TSCv{\tA}{\nA}.south) -- (\TSCv{\tB}{\nB}.south);
    \path[mrttarrow] (\TSCv{\tB}{\nB}.south) -- (\TSCv{\tC}{\nA}.south);
  }

  % An inter-node event on Node A
  \DrawTick{\TSCv{x}{A}}{\TSCv{26}{A}}{\LongTickH}
  \node[textA,text=blue] (\STRv{x}{A}) [below of=\TSCv{x}{A}] {\Tick{c}{x}{A}};

  % Two inter-node events on Node B
  \DrawTick{\TSCv{w}{B}}{\TSCv{12}{B}}{\LongTickH}
  \node[textB] (\STRv{w}{B}) [above of=\TSCv{w}{B}] {\Tick{c}{w}{B}};

  \DrawTick{\TSCv{y}{B}}{\TSCv{20}{B}}{\LongTickH}
  \node[textB] (\STRv{y}{B}) [above of=\TSCv{y}{B}] {\Tick{c}{y}{B}};

  % draw MinRTT
  {
    \xdef\nA{A}
    \xdef\nB{B}
    \xdef\tA{l}
    \xdef\tB{m}
    \xdef\tC{n}
    \xdef\cA{64}
    \xdef\cB{42}
    \xdef\cC{76}

    \DrawTick{\TSCv{\tA}{\nA}}{\TSCv{\cA}{\nA}}{\LongTickH}
    \node[textA] (\STRv{\tA}{\nA}) [below of=\TSCv{\tA}{\nA}]
    {\Tick{c}{\tA}{\nA}};
    \DrawTick{\TSCv{\tC}{\nA}}{\TSCv{\cC}{\nA}}{\LongTickH}
    \node[textA] (\STRv{\tC}{\nA}) [below of=\TSCv{\tC}{\nA}] {\Tick{c}{\tC}{\nA}};
    \DrawTick{\TSCv{\tB}{\nB}}{\TSCv{\cB}{\nB}}{\LongTickH}
    \node[textB] (\STRv{\tB}{\nB}) [above of=\TSCv{\tB}{\nB}] {\Tick{c}{\tB}{\nB}};
    %
    \path (\TSCv{\tA}{\nA}.south) --
    ($(\TSCv{0}{\nB}.south)!(\TSCv{\tA}{\nA})!(\TSCv{1}{\nB}.south)$) coordinate[pos=0]
    (C-MRTT1-bottom-left);
    \path (\TSCv{\tC}{\nA}.south) --
    ($(\TSCv{0}{\nB}.south)!(\TSCv{\tC}{\nA})!(\TSCv{1}{\nB}.south)$) coordinate[pos=1]
    (C-MRTT1-top-right);
    \node[fit=(C-MRTT1-bottom-left) (C-MRTT1-top-right),
    postaction={on layer=back,fill,lightgray!30!white},
    postaction={on layer=back,draw,lightgray!30!white}] (MRTT1-box) {};
    % Round-trip of MRTT#1
    \path[mrttarrow] (\TSCv{\tA}{\nA}.south) -- (\TSCv{\tB}{\nB}.south);
    \path[mrttarrow] (\TSCv{\tB}{\nB}.south) -- (\TSCv{\tC}{\nA}.south);
  }

  % Re-initialize
  \coordinate (AStarts) at (\GlobalX, \YofNodeBCaseB);
  \coordinate (BStarts) at (\GlobalX, \YofNodeCCaseB);
  \coordinate (AEnds) at (\RectW,\YofNodeBCaseB);
  \coordinate (BEnds) at (\RectW,\YofNodeCCaseB);
  \node[rect0,xshift=-5pt] (NodeA) at (AStarts.north) {B};
  \node[rect0,xshift=-5pt] (NodeB) at (BStarts.north) {C};
  \path [timeline,name path=TimelineA] (AStarts) -- (AEnds.west);
  \path [timeline,name path=TimelineB] (BStarts) -- (BEnds.west);

  % All ticks of TSC~C^B
  \edef\X{\GlobalX}
  \edef\name{}
  \foreach \x in {0,1,...,\MaxTksB}
  {
    \xdef\name{\TSCv{\x}{B}}
    \pgfmathparse{\X+\PeriodB}
    \xdef\X{\pgfmathresult}
    \coordinate (\name) at (\X, \YofNodeBCaseB);
    \coordinate[yshift=\SmallTickH] (\name-top) at (\name);
    \path [tick3] (\name.north) -- (\name-top);
  }

  % All ticks of TSC~C^C
  \edef\X{\GlobalX}
  \edef\name{}
  \foreach \x in {0,1,...,\MaxTksC}
  {
    \xdef\name{\TSCv{\x}{C}}
    \pgfmathparse{\X+\PeriodC}
    \xdef\X{\pgfmathresult}
    \coordinate (\name) at (\X, \YofNodeCCaseB);
    \coordinate[yshift=\SmallTickH] (\name-top) at (\name);
    \path [tick3] (\name.north) -- (\name-top);
  }

  % draw MinRTT
  {
    \xdef\nA{B}
    \xdef\nB{C}
    \xdef\tA{o}
    \xdef\tB{p}
    \xdef\tC{q}
    \xdef\cA{1}
    \xdef\cB{14}
    \xdef\cC{7}

    \DrawTick{\TSCv{\tA}{\nA}}{\TSCv{\cA}{\nA}}{\LongTickH}
    \node[textA] (\STRv{\tA}{\nA}) [below of=\TSCv{\tA}{\nA}]
    {\Tick{c}{\tA}{\nA}};
    \DrawTick{\TSCv{\tC}{\nA}}{\TSCv{\cC}{\nA}}{\LongTickH}
    \node[textA] (\STRv{\tC}{\nA}) [below of=\TSCv{\tC}{\nA}] {\Tick{c}{\tC}{\nA}};
    \DrawTick{\TSCv{\tB}{\nB}}{\TSCv{\cB}{\nB}}{\LongTickH}
    \node[textB] (\STRv{\tB}{\nB}) [above of=\TSCv{\tB}{\nB}] {\Tick{c}{\tB}{\nB}};
    %
    \path (\TSCv{\tA}{\nA}.south) --
    ($(\TSCv{0}{\nB}.south)!(\TSCv{\tA}{\nA})!(\TSCv{1}{\nB}.south)$) coordinate[pos=0]
    (C-MRTT1-bottom-left);
    \path (\TSCv{\tC}{\nA}.south) --
    ($(\TSCv{0}{\nB}.south)!(\TSCv{\tC}{\nA})!(\TSCv{1}{\nB}.south)$) coordinate[pos=1]
    (C-MRTT1-top-right);
    \node[fit=(C-MRTT1-bottom-left) (C-MRTT1-top-right),
    postaction={on layer=back,fill,lightgray!30!white},
    postaction={on layer=back,draw,lightgray!30!white}] (MRTT1-box) {};
    % Round-trip of MRTT#1
    \path[mrttarrow] (\TSCv{\tA}{\nA}.south) -- (\TSCv{\tB}{\nB}.south);
    \path[mrttarrow] (\TSCv{\tB}{\nB}.south) -- (\TSCv{\tC}{\nA}.south);
  }

  % An inter-node event on Node B
  \DrawTick{\TSCv{u}{B}}{\TSCv{17}{B}}{\LongTickH}
  \node[textA,text=blue] (\STRv{u}{B}) [below of=\TSCv{u}{B}] {\Tick{c}{u}{B}};

  % An inter-node event on Node C
  \DrawTick{\TSCv{v}{C}}{\TSCv{54}{C}}{\LongTickH}
  \node[textB] (\STRv{v}{C}) [above of=\TSCv{v}{C}] {\Tick{c}{v}{C}};

  % draw MinRTT
  {
    \xdef\nA{B}
    \xdef\nB{C}
    \xdef\tA{r}
    \xdef\tB{s}
    \xdef\tC{t}
    \xdef\cA{39}
    \xdef\cB{95}
    \xdef\cC{43}

    \DrawTick{\TSCv{\tA}{\nA}}{\TSCv{\cA}{\nA}}{\LongTickH}
    \node[textA] (\STRv{\tA}{\nA}) [below of=\TSCv{\tA}{\nA}]
    {\Tick{c}{\tA}{\nA}};
    \DrawTick{\TSCv{\tC}{\nA}}{\TSCv{\cC}{\nA}}{\LongTickH}
    \node[textA] (\STRv{\tC}{\nA}) [below of=\TSCv{\tC}{\nA}] {\Tick{c}{\tC}{\nA}};
    \DrawTick{\TSCv{\tB}{\nB}}{\TSCv{\cB}{\nB}}{\LongTickH}
    \node[textB] (\STRv{\tB}{\nB}) [above of=\TSCv{\tB}{\nB}] {\Tick{c}{\tB}{\nB}};
    %
    \path (\TSCv{\tA}{\nA}.south) --
    ($(\TSCv{0}{\nB}.south)!(\TSCv{\tA}{\nA})!(\TSCv{1}{\nB}.south)$) coordinate[pos=0]
    (C-MRTT1-bottom-left);
    \path (\TSCv{\tC}{\nA}.south) --
    ($(\TSCv{0}{\nB}.south)!(\TSCv{\tC}{\nA})!(\TSCv{1}{\nB}.south)$) coordinate[pos=1]
    (C-MRTT1-top-right);
    \node[fit=(C-MRTT1-bottom-left) (C-MRTT1-top-right),
    postaction={on layer=back,fill,lightgray!30!white},
    postaction={on layer=back,draw,lightgray!30!white}] (MRTT1-box) {};
    % Round-trip of MRTT#1
    \path[mrttarrow] (\TSCv{\tA}{\nA}.south) -- (\TSCv{\tB}{\nB}.south);
    \path[mrttarrow] (\TSCv{\tB}{\nB}.south) -- (\TSCv{\tC}{\nA}.south);
  }

  % Re-initialize
  \coordinate (AStarts) at (\GlobalX, \YofNodeACaseC);
  \coordinate (BStarts) at (\GlobalX, \YofNodeCCaseC);
  \coordinate (AEnds) at (\RectW,\YofNodeACaseC);
  \coordinate (BEnds) at (\RectW,\YofNodeCCaseC);
  \node[rect0,xshift=-5pt] (NodeA) at (AStarts.north) {A};
  \node[rect0,xshift=-5pt] (NodeB) at (BStarts.north) {C};
  \path [timeline,name path=TimelineA] (AStarts) -- (AEnds.west);
  \path [timeline,name path=TimelineB] (BStarts) -- (BEnds.west);

  % All ticks of TSC~C^A
  \edef\X{\GlobalX}
  \edef\name{}
  \foreach \x in {0,1,...,\MaxTksA}
  {
    \xdef\name{\TSCv{\x}{A}}
    \pgfmathparse{\X+\PeriodA}
    \xdef\X{\pgfmathresult}
    \coordinate (\name) at (\X, \YofNodeACaseC);
    \coordinate[yshift=\SmallTickH] (\name-top) at (\name);
    \path [tick3] (\name.north) -- (\name-top);
  }

  % All ticks of TSC~C^C
  \edef\X{\GlobalX}
  \edef\name{}
  \foreach \x in {0,1,...,\MaxTksC}
  {
    \xdef\name{\TSCv{\x}{C}}
    \pgfmathparse{\X+\PeriodC}
    \xdef\X{\pgfmathresult}
    \coordinate (\name) at (\X, \YofNodeCCaseC);
    \coordinate[yshift=\SmallTickH] (\name-top) at (\name);
    \path [tick3] (\name.north) -- (\name-top);
  }

  % draw MinRTT
  {
    \xdef\nA{A}
    \xdef\nB{C}
    \xdef\tA{a}
    \xdef\tB{b}
    \xdef\tC{c}
    \xdef\cA{2}
    \xdef\cB{12}
    \xdef\cC{14}

    \DrawTick{\TSCv{\tA}{\nA}}{\TSCv{\cA}{\nA}}{\LongTickH}
    \node[textA] (\STRv{\tA}{\nA}) [below of=\TSCv{\tA}{\nA}]
    {\Tick{c}{\tA}{\nA}};
    \DrawTick{\TSCv{\tC}{\nA}}{\TSCv{\cC}{\nA}}{\LongTickH}
    \node[textA] (\STRv{\tC}{\nA}) [below of=\TSCv{\tC}{\nA}] {\Tick{c}{\tC}{\nA}};
    \DrawTick{\TSCv{\tB}{\nB}}{\TSCv{\cB}{\nB}}{\LongTickH}
    \node[textB] (\STRv{\tB}{\nB}) [above of=\TSCv{\tB}{\nB}] {\Tick{c}{\tB}{\nB}};
    %
    \path (\TSCv{\tA}{\nA}.south) --
    ($(\TSCv{0}{\nB}.south)!(\TSCv{\tA}{\nA})!(\TSCv{1}{\nB}.south)$) coordinate[pos=0]
    (C-MRTT1-bottom-left);
    \path (\TSCv{\tC}{\nA}.south) --
    ($(\TSCv{0}{\nB}.south)!(\TSCv{\tC}{\nA})!(\TSCv{1}{\nB}.south)$) coordinate[pos=1]
    (C-MRTT1-top-right);
    \node[fit=(C-MRTT1-bottom-left) (C-MRTT1-top-right),
    postaction={on layer=back,fill,lightgray!30!white},
    postaction={on layer=back,draw,lightgray!30!white}] (MRTT1-box) {};
    % Round-trip of MRTT#1
    \path[mrttarrow] (\TSCv{\tA}{\nA}.south) -- (\TSCv{\tB}{\nB}.south);
    \path[mrttarrow] (\TSCv{\tB}{\nB}.south) -- (\TSCv{\tC}{\nA}.south);
  }

  % An inter-node event on Node C
 %\DrawTick{\TSCv{z}{C}}{\TSCv{68}{C}}{\LongTickH}
 %\node[textB] (\STRv{z}{C}) [above of=\TSCv{z}{C}] {\Tick{c}{z}{C}};

  % draw MinRTT
  {
    \xdef\nA{A}
    \xdef\nB{C}
    \xdef\tA{d}
    \xdef\tB{e}
    \xdef\tC{f}
    \xdef\cA{66}
    \xdef\cB{93}
    \xdef\cC{77}

    \DrawTick{\TSCv{\tA}{\nA}}{\TSCv{\cA}{\nA}}{\LongTickH}
    \node[textA] (\STRv{\tA}{\nA}) [below of=\TSCv{\tA}{\nA}]
    {\Tick{c}{\tA}{\nA}};
    \DrawTick{\TSCv{\tC}{\nA}}{\TSCv{\cC}{\nA}}{\LongTickH}
    \node[textA] (\STRv{\tC}{\nA}) [below of=\TSCv{\tC}{\nA}] {\Tick{c}{\tC}{\nA}};
    \DrawTick{\TSCv{\tB}{\nB}}{\TSCv{\cB}{\nB}}{\LongTickH}
    \node[textB] (\STRv{\tB}{\nB}) [above of=\TSCv{\tB}{\nB}] {\Tick{c}{\tB}{\nB}};
    %
    \path (\TSCv{\tA}{\nA}.south) --
    ($(\TSCv{0}{\nB}.south)!(\TSCv{\tA}{\nA})!(\TSCv{1}{\nB}.south)$) coordinate[pos=0]
    (C-MRTT1-bottom-left);
    \path (\TSCv{\tC}{\nA}.south) --
    ($(\TSCv{0}{\nB}.south)!(\TSCv{\tC}{\nA})!(\TSCv{1}{\nB}.south)$) coordinate[pos=1]
    (C-MRTT1-top-right);
    \node[fit=(C-MRTT1-bottom-left) (C-MRTT1-top-right),
    postaction={on layer=back,fill,lightgray!30!white},
    postaction={on layer=back,draw,lightgray!30!white}] (MRTT1-box) {};
    % Round-trip of MRTT#1
    \path[mrttarrow] (\TSCv{\tA}{\nA}.south) -- (\TSCv{\tB}{\nB}.south);
    \path[mrttarrow] (\TSCv{\tB}{\nB}.south) -- (\TSCv{\tC}{\nA}.south);
  }

  %Newtonian Time
  \coordinate[yshift=-48pt] (C-NewtonTime-west) at (AStarts);
  \coordinate[yshift=-48pt] (C-NewtonTime-east) at (AEnds);
  \path [>=Latex,->,draw=yellow!75!magenta,line width=2.0\pgflinewidth,name path=NewtonTime]
  (C-NewtonTime-west) -- (C-NewtonTime-east) coordinate[pos=0.808,yshift=-8pt] (C-NewtonTime);
  \node (S-NewtonTime) at (C-NewtonTime) {Newtonian Time};
\end{scope}
\end{tikzpicture}

